RODE-Net: Learning Ordinary Differential Equations with Randomness from Data

Random ordinary differential equations (RODEs), i.e. ODEs with random parameters, are often used to model complex dynamics. Most existing methods to identify unknown governing RODEs from observed data often rely on strong prior knowledge. Extracting the governing equations from data with less prior knowledge remains a great challenge. In this paper, we propose a deep neural network, called RODE-Net, to tackle such challenge by fitting a symbolic expression of the differential equation and the distribution of parameters simultaneously. To train the RODE-Net, we first estimate the parameters of the unknown RODE using the symbolic networks \cite{long2019pde} by solving a set of deterministic inverse problems based on the measured data, and use a generative adversarial network (GAN) to estimate the true distribution of the RODE's parameters. Then, we use the trained GAN as a regularization to further improve the estimation of the ODE's parameters. The two steps are operated alternatively. Numerical results show that the proposed RODE-Net can well estimate the distribution of model parameters using simulated data and can make reliable predictions. It is worth noting that, GAN serves as a data driven regularization in RODE-Net and is more effective than the $\ell_1$ based regularization that is often used in system identifications.

==> section2-liujunyu.tex <==
\section{The RODE-Net framework}
Given a set of observed time series data $\{x(t)\} \subset \mathbb{R}^d$ with $d$ being the dimension of the observable quantities, we aim to discover the governing RODE from the data. We assume that the RODE to be discovered takes the following form:
\begin{equation}
    \frac{dx}{dt} = F_\eta(x, t),{\color{red}x\in\mathbb{R}^d,t\geq0}
\end{equation}
where $F(\cdot): \mathbb{R}^{d+1}\to\mathbb{R}^d$ is a $d$ dimensional vector function and $\eta \sim \mathcal{P}(\eta)$ is the random parameter of $F$. 
The RODE actually describes a set of ODEs determined by the random parameter $\eta$.
For each sampled $\eta$, e.g., $\eta_i$, we call the associated ODE as ODE-$\eta_i$.
% {\color{blue} For each sampled $\eta$, e.g., $\eta_i$, we call this specific ODE as ODE-$\eta_i$.}
% add: ODE eta_i sample from RODE
%
We note that the RODEs in this paper are different from those considered in 
\cite{han2017random,neckel2013random}. The latter consider system parameters
as random processes (e.g. solution of SDE) rather than the random variables, 
which results in solutions with higher regularity. 
% To our best of knowledge, most related researches such as\cite{grune2001pathwise,asai2016multi,kloeden2007pathwise,asai2013stable,asai2013numerical,asai2016numerical} work on designing efficient numerical schemes instead of inverse problems. 

% [在这里加上RODE的概念解释]

\begin{figure}[htbp!]
		\centering
		\includegraphics[width = 0.8\textwidth]{pic/RODEnet_structure.png}
		\caption{The structure of RODE-Net}\label{fig:RODE-net}
\end{figure}

% {\color{green} The observed data are sampled from several deterministic ODEs with the same form while the realizations of $\eta$ remain unknown. }
The observed data of an RODE are correlated with a set of underlying ODE-$\eta_i$s while the $\eta_i$s remain unknown.
% {\color{blue} We sample a set of ODE-$\eta_i$ and the observed data can be generated from numerical simulations of these ODEs.}
%
% estimate the support and distribution
% {\color{green} Our proposed RODE-Net (Fig. \ref{fig:RODE-net}) is designed to identify the deterministic ODEs and the RODE at the same time. }
Our proposed RODE-Net (Fig. \ref{fig:RODE-net}) is designed to identify the ODE-$\eta_i$s separately and to estimate the distribution of $\eta$ at the same time.
To achieve both objectives, the RODE-Net framework is consisted of two main components: the GAN and the ODE-Net which is based on the SymNet. 
% 跟前面的说法保持统一

Each component will be introduced by detail in the following subsections. 
In general, the ODE-Net solves a deterministic inverse problem and estimates each ODE-$\eta_i$ from observed data,
% 解确定性反问题 引出odenet
and the GAN learns the distribution of $\eta_i$s from the parameters of ODE-Nets. 
The GAN eventually represents the estimated RODE and is able to generate ODEs with randomness.
Moreover, we address that the GAN can also work as an ideal regularization in training ODE-Net.
% ref figure 1

\subsection{ODE-Net}

% {\color{green} The ODE-Net is a parameterized representation of an ODE and is consisted of several SymNets. Each SymNet represents a component of the vector function $F$. }
The ODE-Net can learn a parameterized representation of an ODE which takes the following form
\begin{equation}
\frac{dx}{dt} = F(x, t), x\in\mathbb{R}^d, t\geq0.
\end{equation}
The ODE-Net is a reduced version of PDE-Net 2.0\cite{long2019pde} and only contains several SymNets to approximate each component of the right-hand multivariate nonlinear vector function $F$ of an ODE.

% the SymNet: function and structure
As is introduced in PDE-Net 2.0, the SymNet is a symbolic neural network which can approximate polynomials of variables and is able to output the expression of the equation through symbolic computation. There are two hyper-parameters to characterize the structure of a SymNet: 
\begin{enumerate}
    \item the dimension of the input $d$, which equals to the dimension of $x$ in ODE-Net;
    \item the number of hidden layers $k$, which determines the expression power of the SymNet.
\end{enumerate}

% the delta t block concept
Similar to PDE-Net 2.0, the ODE-Net adopts the forward Eular discretization in time space and inherits the concept of $\delta t$-block. One $\delta t$-block means making prediction in one time unit, which is given by
\begin{equation}
    \hat{\mathbf{x}}_i(t+\delta t) \approx \hat{\mathbf{x}}_i(t) + \delta t \cdot SymNet_d^k(\hat{\mathbf{x}}), \label{deltat_block_ode}
\end{equation}
and a long-term prediction can be realized by stacking multiple $\delta t$-blocks recurrently. Fig. \ref{fig:ODE-net} shows the structure of $\delta t$-blocks and the ODE-Net.

\begin{figure}[htbp!]
		\centering
		\includegraphics[width = 0.8\textwidth]{pic/ODE-Net_structure.png}
		\caption{The structure of RODE-Net}\label{fig:ODE-net}
\end{figure}

% [add details of ODE-Net/SymNet(figure)]
% {\color{blue}
% The ODE-Net is a reduced version of PDE-Net 2.0\cite{long2019pde} and the 
% architecture of ODE-Net can be read as the following simple form

% }

\subsection{The GAN component}
% GAN在我们这里的作用
The GAN in RODE-Net aims to learn the distribution of parameters of ODEs and thus can represent the underlying RODE. The learned GAN can further work as a regularization to better train an ODE-Net as it provides additional information of the RODE which is beyond the observed data.

% 介绍GAN 写一下minmax的问题
The specific type of GAN we adopt is WGAN (Wasserstein GAN \cite{arjovsky2017wasserstein,gulrajani2017improved}), which is easier to train compared to the traditional GAN \cite{goodfellow2014generative}. The GAN usually contains a generator $G$ and a discriminator $D$ and the traditional GAN optimizes over the following problem
\begin{equation}
    \min_G \max_D \mathbb{E}_{\mathbf{x} \sim p_r} \log [ D(\mathbf{x}) ] + \mathbb{E}_{\mathbf{z} \sim p_{\mathbf{z}}} \log [1-D(G(\mathbf{z}))],
\end{equation}
where $p_r$ is the distribution of the real data and $p_z$ is the prior distribution of the input of $G$.
The WGAN proposes to use the Wasserstein distance to describe the difference between two distributions, which is formulated as follows:
\begin{equation}
W(p_{r}, p_{g}) = \sup_{||f||_L \leq 1} \mathbb{E}_{x\sim p_r} f(x) - \mathbb{E}_{x\sim p_g}f(x), \label{Wdist}
\end{equation}
where $p_g$ is the distribution of data generated by $G$.
The discriminator in WGAN approximates the $f(\cdot)$ in \eqref{Wdist} and the WGAN optimizes over the following constrained problem:
\begin{equation}
    \min_G \max_D \mathbb{E}_{\mathbf{x} \sim p_r} D(\mathbf{x}) - \mathbb{E}_{\mathbf{z} \sim 
    p_{\mathbf{z}}} D(G(\mathbf{z})) 
    \quad s.t. ||D||_L \leq 1.
\end{equation}

% 我们用的具体网络结构
In RODE-Net, $G$ and $D$ are neural networks with multiple fully connected hidden layers and non-linear activations. The structure of the generator and discriminator is shown in [fig/table].




==> section3-liujunyu.tex <==
\section{Training strategy}
The training of RODE-Net is multistage. First we train the ODE-Nets with observed data to obtain numbers of ODE-Nets which well describe the observations. Then we train the GAN on the fitted ODE-Nets to obtain the distribution. Finally the GAN can be used to finetune or train new ODE-Nets as a regularization instead of L1.

\subsection{Stage-0} \label{sec:stage-0}
% main: 
% 1. one ODE-Net matches one ODE
% 2. data loss + sparsity loss
% 3. multi-step training strategy

At the first stage (stage-0), we aim to figure out the ODEs lying behind the observed data. 
Suppose the data are collected as follows:
\begin{enumerate}
    \item Sample multiple ODEs marked as $F_{\eta_i}$ from one RODE;
    \item For the $i$-th ODE, one or more initial states $x_i^j(0)$ may be given;
    \item For the $j$-th initial state of the $i$-th ODE,  we can acquire a set of consequent states ${x_i^j(t)}$ evolving from it.
\end{enumerate}

Since the data are collected from multiple ODEs, we need multiple ODE-Nets to fit them, and the training of different ODE-Nets can be done separately. The loss function we used to train one ODE-Net is
\begin{equation}
    L_{\text{odenet}}(\xi_i, \mathbf{x}_i(t)) =
    L_{\text{data}}(\xi_i, \mathbf{x}_i(t)) + 
    \lambda_s L_{\text{sparsity}}(\xi_i)
    \label{odenet_loss},
\end{equation}
where the data loss term 
\begin{equation}
    L_{\text{data}}(\xi_i, \mathbf{x}_i(t)) = 
    \frac{1}{N_i}
    \sum_{j=1}^{N_i} \sum_{k=1}^{T_j} 
    w_k ||\hat{\mathbf{x}}_{\xi_i}(t_k)-\mathbf{x}_i^j(t_k)||_2^2 / \delta t^2 
    \label{data_loss}
\end{equation}
describes the accuracy of the ODE to match the data, and the sparsity loss term
\begin{equation}
    L_{\text{sparsity}}(\xi_i) = 
    \sum_{j=1}^{l} l_s(\xi_i^{(j)})
    \label{sparse_loss}
\end{equation}
is to encourage the ODE to have a sparse form for better interpretability, and 
\begin{equation}
    l_s(p) = \begin{cases}
    |p| - \frac{s}{2} & \text{if \,}  |p|>s \\
    \frac{1}{2s}p^2 & \text{else}
    \end{cases}
    \label{huber_loss}
\end{equation}
is the Huber loss function, i.e. a smoothed L1 loss.

The ODE-Net can give prediction of multi steps with given initial value $x(0)$ using multiple $\delta t$-blocks, we adopt a strategy to gradually increase the number of steps when training. This strategy is to ensure the accuracy of long-term prediction and to keep the model stable during training.

The algorithm to train one ODE-Net is given in \ref{alg:pretrain}.

\begin{algorithm}
\caption{Stage-0 (pretrain ODE-Net): pretrain($\xi, \mathbf{x}(t)$)}
\label{alg:pretrain}
\begin{algorithmic}[1]

\FOR{$s$=1,...,$s_{max}$}
\WHILE{$\xi$ has not converged}
    \STATE Sample $m$ subsequences from all the subsequences of $\mathbf{x}(t)$ with length $s+1$, thus we have a batch of training data $\{\mathbf{x}^j(0), ..., \mathbf{x}^j(s)\}_{j=1}^m$;
    \STATE Do the forward computation: let $\hat{\mathbf{x}}^j(0) = \mathbf{x}^j(0)$, and compute $\hat{\mathbf{x}}^j(t+1) = Net_{\xi}(\hat{\mathbf{x}}^j(t)), t=1,...,s, j=1,...,m$
    \STATE Calculate the loss on the batch data
    \begin{equation*}
        L = \frac{1}{m}\sum_{i=1}^m \sum_{t=1}^{s} w_t ||\hat{\mathbf{x}}^j(t)-\mathbf{x}^j(t)||_2^2 + \lambda_s L_{\text{sparsity}}(\xi)
    \end{equation*}
    \STATE Calculate the gradient $\nabla_\xi L$ and update the parameters $\xi$ using Adam.
\ENDWHILE
\ENDFOR
\end{algorithmic}
\end{algorithm}

\subsection{Stage-1}

We flatten the parameters of each ODE-Net to a vector to form the training data of the GAN. Note that these parameter vectors are not real data of common sense (the true ODE that the observed data come from), but an estimation of real data. The parameter vectors can be noisy and inaccurate due to the training error in stage-0.
When training the GAN, we update G and D alternatively by convention and optimize over the WGAN-GP loss. The training algorithm is given in \ref{alg:WGAN}.

\begin{algorithm}
\caption{Stage-1 (training GAN): trainGAN($\theta, V, \Xi$)}
\label{alg:WGAN}
\begin{algorithmic}[1]

\WHILE{$\theta$ has not converged}
    
    \FOR{Iteration of discriminator $n_d$}
    
    \STATE Sample $\{\mathbf{z}^{(1)}, ..., \mathbf{z}^{(m)}\}$ a batch from the prior $p(\mathbf{z})$;
    \STATE Sample $\{\mathbf{\xi}^{(1)}, ..., \mathbf{\xi}^{(m)}\}$ a batch from the parameter vectors of trained ODE-Nets $\Xi$;
    \STATE Sample $\{\epsilon^{(1)}, ..., \epsilon^{(m)}\}$ from $U[0,1]$;
    \STATE Let $\hat{\xi}^{(i)}=G_\theta(\mathbf{z}^{(i)}),  \tilde{\xi}^{(i)} = \epsilon^{(i)}\xi^{(i)} + (1-\epsilon^{(i)}) \hat{\xi}^{(i)}, i=1, ..., m$;
    \STATE Calculate the WGAN-GP loss by
    \begin{equation*}
         L = \frac{1}{m}\sum_{i=1}^m \left[ 
         D_V(\hat{\xi}^{(i)}) - 
         D_V(\mathbf{\xi}^{(i)}) +
         \lambda (||\nabla_{\hat{\xi}^{(i)}} D_V(\tilde{\xi}^{(i)}) ||_2-1)^2
         \right],
    \end{equation*}
    \STATE Update $V$ using Adam with gradient descent.
    \ENDFOR
    
    \STATE Sample $\{\mathbf{z}^{(1)}, ..., \mathbf{z}^{(m)}\}$ from the prior $p(\mathbf{z}))$;
    \STATE Calculate the gradient of the generator`s parameter $\theta$ by
    \begin{equation*}
        - \nabla_{\theta} \frac{1}{m}\sum_{i=1}^m D_V(G_\theta(\mathbf{z}^{(i)}))
    \end{equation*}
    \STATE Update $\theta$ using Adam with gradient descent.
\ENDWHILE
\end{algorithmic}
\end{algorithm}


\subsection{Stage-2}
In this stage, we update the ODE-Nets and the GAN alternatively. The GAN now works as a regularization in training ODE-Nets to provide the knowledge of the underlying RODE and to help correct the training error of ODE-Net. For each ODE-Net, not only the corresponding observed data are available, it can also make use of the global information passed from GAN, which has captured the distribution of all ODE-Nets. The GAN connects all ODE-Nets and makes the ODE-Nets not alone anymore.

In addition to the data loss term and the sparsity loss term introduced in section \ref{sec:stage-0}, we have another loss term namely the GAN regularization, which is simply formulated as
\begin{equation}
    L_{GANreg}(\xi) = D_V(\xi).
\end{equation}
The GAN regularization is actually switching the role of the generator and the ODE-Nets and pushing the parameters of the ODE-Nets to be similar to what can be generated by the learned generator. The full loss used in stage-2 to update an ODE-Net is
\begin{equation}
    L_{odenet}^{stage2} (\xi, x(t)) = L_{data}(\xi, x(t)) + \lambda_s L_{sparsity}(\xi) + \lambda_G L_{GANreg}(\xi).
\end{equation}
 
The alternating of updating the ODE-Nets and GAN in this stage is a mixing procedure of stage-0 and stage-1, except that we have modified the loss of training ODE-Nets. This algorithm is detailed in \ref{alg:stage2}.

\begin{algorithm}
\caption{Stage-2 (updating ODE-Nets and the GAN alternatively): trainStage2($\theta, V, \Xi$, x(t))}.
\label{alg:stage2}
\begin{algorithmic}[1]

\WHILE{$\Xi$ has not converged}
    \FOR{i=1,...,$N_E$}
    \STATE Update the $i$-th ODE-Net using $L_{odenet}^{stage2} (\xi_i, x_i(t))$ ;
    \FOR{Iteration of discriminator $n_{d}^{stage2}$}
    \STATE Update the discriminator $D_V$ using WGAN-GP loss ;
    \ENDFOR
    \ENDFOR
    \FOR{Iteration of GAN $n_{GAN}^{stage2}$}
    \STATE trainGAN($\theta, V, \Xi$);
    \ENDFOR
\ENDWHILE
\end{algorithmic}
\end{algorithm}



